Revisiting the Learned Clauses Database Reduction Strategies

In this paper, we revisit an important issue of CDCL-based SAT solvers, namely the learned clauses database management policies. Our motivation takes its source from a simple observation on the remarkable performances of both random and size-bounded reduction strategies. We first derive a simple reduction strategy, called Size-Bounded Randomized strategy (in short SBR), that combines maintaing short clauses (of size bounded by k), while deleting randomly clauses of size greater than k. The resulting strategy outperform the state-of-the-art, namely the LBD based one, on SAT instances taken from the last SAT competition. Reinforced by the interest of keeping short clauses, we propose several new dynamic variants, and we discuss their performances.

==> defs.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Definition de nouvelles commandes % 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\stc}[1]{\mbox{$\langle\,#1\/\, \rangle$}}
\newcommand{\cro}[1]{\mbox{$\[\,#1\/ \]$}}
\newcommand{\ens}[1]{\mbox{$\{\,#1\/\,\}$}}
\newcommand{\quo}[1]{``#1''}
\newcommand{\egaldef}{\mbox{$\stackrel{\rm def}{=}$}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Definition de symboles logiques utiles %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% symboles de BI

\newcommand{\BImtop}{I} % unite conjonctive multiplicative 
\newcommand{\BIatop}{\top} % unite conjonctive additive
\newcommand{\BIabot}{\bot} % unite disjonctive additive
\newcommand{\BImand}{\ast} % conjonction multiplicative
\newcommand{\BImimp}{-\hspace{-1ex}\ast} % implication multiplicative
\newcommand{\BIaand}{\wedge} % conjonction additive
\newcommand{\BIaimp}{\rightarrow} % implication additive
\newcommand{\BIaor}{\vee} % disjonction additive
\newcommand{\BImnul}{\emptyset_m} % bunch multiplicatif vide
\newcommand{\BIanul}{\emptyset_a} % bunch additif vide
\newcommand{\BIax}{ax} % nom de la regle axiome
\newcommand{\BIcut}{cut} % nom de la regle de coupure
\newcommand{\BIweak}{w} % nom de la regle d'affaiblissement
\newcommand{\BIcont}{c} % nom de la regle de contraction
\newcommand{\BIequi}{\equiv} % nom de la regle d'equivalence structurelle

\newcommand{\BIvarp}{L} % lettre pour l'ensemble de variables propositionnelles

%\BIprop[varprop]: ensemble des propositions de BI issues de varprop
\newcommand{\BIprop}[1][\BIvarp]{{\cal P}({#1})}

% symboles de MILL

\newcommand{\LLtimes}{\otimes}
\newcommand{\LLwith}{\&}
\newcommand{\LLpar}{\rotatebox[origin=c]{180}{\rm \LLwith}}
\newcommand{\LLimp}{-\hspace{-1ex}\circ}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Definition d'abbreviations utiles %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\IL}{{\bf IL}}
\newcommand{\LL}{{\bf LL}}
\newcommand{\MLL}{{\bf MLL}}
\newcommand{\ILL}{{\bf ILL}}
\newcommand{\MILL}{{\bf MILL}}
\newcommand{\BIc}{{\bf \BI$^{\bot}$}}
\newcommand{\BI}{{\bf BI}}
\newcommand{\TBI}{{\bf TBI}}
\newcommand{\NBI}{{\bf NBI}}
\newcommand{\NBIA}{\NBI$^{\heartsuit}$}
\newcommand{\LBI}{{\bf LBI}}
\newcommand{\LBIc}{{\bf LBI$^{\bot}$}}
\newcommand{\LBIA}{\LBI$^{\heartsuit}$}
\newcommand{\KRM}{{\bf Krm}}
\newcommand{\KRMs}{{\bf Krms}}
\newcommand{\KRI}{{\bf Kri}}
\newcommand{\KRIs}{{\bf Kris}}
\newcommand{\bunch}{\quo{bunch}}
\newcommand{\bunches}{\quo{bunches}}
\newcommand{\Bunch}{\quo{Bunch}}
\newcommand{\Bunches}{\quo{Bunches}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Macros pour dessiner les sequents %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% consequences syntaxiques |-

\newcommand{\seq}[3][]{\mbox{${#2}\vdash_{#1}{#3}$}}
\newcommand{\seqBI}[2]{\seq[BI]{#1}{#2}}
\newcommand{\seqIL}[2]{\seq[IL]{#1}{#2}}
\newcommand{\seqMILL}[2]{\seq[MILL]{#1}{#2}}

\newcommand{\notseq}[3][]{\mbox{${#2}\not\vdash_{#1}{#3}$}}
\newcommand{\notseqBI}[2]{\notseq[BI]{#1}{#2}}
\newcommand{\notseqIL}[2]{\notseq[IL]{#1}{#2}}
\newcommand{\notseqMILL}[2]{\notseq[MILL]{#1}{#2}}

% consequences semantiques |=

\newcommand{\csm}[3][]{\mbox{${#2}\models_{#1}{#3}$}}
\newcommand{\csmBI}[2]{\csm[BI]{#1}{#2}}
\newcommand{\csmIL}[2]{\csm[IL]{#1}{#2}}
\newcommand{\csmMILL}[2]{\csm[MILL]{#1}{#2}}

\newcommand{\notcsm}[3][]{\mbox{${#2}\not\models_{#1}{#3}$}}
\newcommand{\notcsmBI}[2]{\notcsm[BI]{#1}{#2}}
\newcommand{\notcsmIL}[2]{\notcsm[IL]{#1}{#2}}
\newcommand{\notcsmMILL}[2]{\notcsm[MILL]{#1}{#2}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Notations pour les structures semantiques %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\wld}[1][m]{#1} % lettre pour un monde
\newcommand{\Wld}[1][M]{#1} % lettre pour un ensemble de mondes

\newcommand{\krm}[1][M]{{\cal #1}} % lettre pour un KRM
\newcommand{\kri}[1][I]{{\cal #1}} % lettre pour une KRI=KRM+forcing
\newcommand{\ronb}[1][\bullet]{#1} % lettre pour l'operation de composition
\newcommand{\neus}[1][e]{#1} % lettre pour l'element neutre

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Notations pour les labels %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\neu}[1][1]{#1} % lettre pour l'element neutre
\newcommand{\ron}[1][\circ]{#1} % lettre pour l'operation de composition

\newcommand{\cst}[1][c]{#1} % lettre pour une constante
\newcommand{\Cst}[1][C]{#1} % ensemble de constantes
\newcommand{\Csti}[2][\Cst]{#1_{#2}}

\newcommand{\var}[1][v]{#1} % lettre pour une variable
\newcommand{\Var}[1][V]{#1} % lettre pour un ensemble de variables
\newcommand{\Vari}[2][\Var]{#1_{#2}}

\newcommand{\C}{\mathrm{\Cst}}
\newcommand{\CV}{\mathrm{\Cst\Var}}
\newcommand{\CVi}[1]{\mathrm{\Csti{#1}\Vari{#1}}}

\newcommand{\clos}[1]{\overline{#1}}

\newcommand{\lap}[1][P]{\mathrm{#1}} % lettre pour un alphabet propositionnel
\newcommand{\PROP}[1][{{\cal P}}]{#1} % langage propositionnel
\newcommand{\PROPi}[2][\PROP]{#1_{#2}}
\newcommand{\Prop}[1][P]{#1} % ensemble de propositions
\newcommand{\Propi}[2][\Prop]{#1_{#2}}

\newcommand{\lal}[1][L]{\mathrm{#1}} % lettre pour un alphabet de labels
\newcommand{\LAB}[1][{{\cal L}}]{#1} % langage de labels
\newcommand{\LABi}[2][\LAB]{#1_{#2}}
\newcommand{\LABC}[1][{\clos{\cal L}}]{#1} % langage de labels
\newcommand{\LABCi}[2][\LABC]{#1_{#2}}

\newcommand{\lab}[1][l]{#1} % lettre pour un label
\newcommand{\Lab}[1][L]{#1} % ensemble de labels
\newcommand{\Labi}[2][\Lab]{#1_{#2}}

\newcommand{\kon}[1][k]{#1} % lettre pour une contrainte
\newcommand{\Kon}[1][K]{#1} % ensemble de contraintes
\newcommand{\Koni}[2][\Kon]{#1_{#2}} % ensemble de contraintes
\newcommand{\KON}[1][{{\cal K}}]{#1} % langage de contraintes
\newcommand{\KONi}[2][\KON]{#1_{#2}} % langage de contraintes
\newcommand{\KONC}[1][{\clos{\cal K}}]{#1} % langage de contraintes
\newcommand{\KONCi}[2][\KONC]{#1_{#2}} % langage de contraintes

\newcommand{\KLi}[1]{\LAB\KONi{\mathrm{#1}}}

\newcommand{\K}{\Kon}
\newcommand{\Ki}[1]{\Kon_{#1}}

\newcommand{\Laa}[1][{{\cal L}}]{\widetilde{#1}} % algebre de labels
\newcommand{\Laai}[2][\Laa]{#1_{#2}} % algebre de labels

\newcommand{\kleqs}{\sqsubseteq} % symbole d'ordre plus petit que
\newcommand{\kleq}{\leq} % symbole d'ordre plus petit que
\newcommand{\kgeq}{\geq} % symbole d'ordre plus grand que

\newcommand{\ass}[1][as]{#1} % lettre pour une assertion
\newcommand{\Ass}[1][As]{#1} % lettre pour un ensemble d'assertions
\newcommand{\Assi}[2][\Ass]{#1_{#2}} % lettre pour un ensemble d'assertions
\newcommand{\AssC}[1][{\clos{\Ass}}]{#1}

\newcommand{\obl}[1][rq]{#1} % lettre pour  une obligation
\newcommand{\Obl}[1][Rq]{#1} % lettre pour un ensemble d'obligations
\newcommand{\Obli}[2][\Obl]{#1_{#2}} % lettre pour un ensemble d'obligations

% \kontr[nom]{label1}{label2} fabrique une contrainte 'l1<=l2' 
\newcommand{\kontr}[3][\kleq]{\mbox{$#2#1#3$}}
\newcommand{\kontrb}[3][\kleq]{\fbox{$#2#1#3$}}

\newcommand{\kontrs}[3][\kleqs]{\mbox{$#2#1#3$}}
\newcommand{\kontrsb}[3][\kleqs]{\fbox{$#2#1#3$}}

% \asser[indice]{l1}{l2} fabrique une assertion ICindice: l1 <= l2
\newcommand{\asser}[3][]{\kontr{\ass_{#1}:#2}{#3}}

% \asserb[indice]{l1}{l2} fabrique une assertion ICindice: l1 <= l2 et
%                         met cette assertion dans une boite
\newcommand{\asserb}[3][]{\kontrb{\ass_{#1}:#2}{#3}}

% \oblig[indice]{l1}{l2} fabrique une obligation RCindice: l1 <= l2
\newcommand{\oblig}[3][]{\kontr{\obl_{#1}:#2}{#3}}

% \obligb[indice]{l1}{l2} fabrique une obligation RCindice: l1 <= l2 et
%                         met cette obligation dans une boite
\newcommand{\obligb}[3][]{\kontrb{\obl_{#1}:#2}{#3}}

\newcommand{\LHS}[1]{LHS(#1)}

\newcommand{\RHS}[1]{RHS(#1)}


\newcommand{\subl}{\prec}
\newcommand{\subleq}{\preceq}
\newcommand{\Sublab}{{\cal P}}
\newcommand{\reml}{\backslash}
\newcommand{\garrow}{\rightarrowtriangle}
\newcommand{\qqquad}{\quad\quad\quad}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Notations pour les propositions %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% lettres pour nommer les variables propositionnelles
\newcommand{\vp}[1][A]{#1}
\newcommand{\vpA}[1][A]{#1}
\newcommand{\vpB}[1][B]{#1}
\newcommand{\vpC}[1][C]{#1}
\newcommand{\vpD}[1][D]{#1}
\newcommand{\vpE}[1][E]{#1}

% lettres pour nommer les meta-variables propositionnelles
\newcommand{\VP}[1][A]{#1}
\newcommand{\VPX}[1][X]{#1}
\newcommand{\VPA}[1][A]{#1}
\newcommand{\VPB}[1][B]{#1}
\newcommand{\VPC}[1][C]{#1}
\newcommand{\VPD}[1][D]{#1}
\newcommand{\VPE}[1][E]{#1}


% \fl{formule}{label} fabrique une formule labellisee
\newcommand{\fl}[2]{\mbox{${#1}:{#2}$}}

% \fls{polarite}{formule}{label} fabrique une formule polarisee labellisee 
\newcommand{\fls}[3]{\mbox{$#1\;\fl{#2}{#3}$}} 

% lettre pour un ensemble de formules polarisees labellisees
\newcommand{\Fls}[1][{{\cal F}}]{#1} 
\newcommand{\Flsi}[2][\Fls]{#1_{#2}}

% \cnx{formule}{label_T}{label_F}: ecriture d'une connexion
\newcommand{\cnx}[3]{\stc{\fls{T}{#1}{#2},\fls{F}{#1}{#3}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Notations diverses                   %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\ett}[1][Es]{#1} % lettre pour les etats
\newcommand{\Ett}[1][{{\cal S}}]{#1} % lettre pour les ensembles d'etats 
\newcommand{\Etti}[2][\Ett]{#1_{#2}} % lettre pour les ensembles d'etats 

\newcommand{\cfg}[1][t]{#1} % lettre pour une configuration
\newcommand{\Cfg}[1][{{\cal T}}]{#1} % ensemble de configurations (tableau)
\newcommand{\Cfgi}[2][\Cfg]{#1_{#2}} % ensemble de configurations (tableau)

% \conf{Etats}{Cst}{Var}{Ass}{0bl} fabrique une configuration
\newcommand{\confs}[4]{\stc{#1,#2,#3,#4}} 

% \conf{Etats}{Cst}{Var}{Ass}{0bl} fabrique une configuration
\newcommand{\conf}[5]{\stc{#1,#2,#3,#4,#5}} 

\newcommand{\sig}[1][\sigma]{#1} % lettre pour une valuation
\newcommand{\Sig}[1][\Sigma]{#1} % ensemble de valuations
\newcommand{\Sigi}[2][\Sig]{#1_{#2}} % ensemble de valuations

\newcommand{\ome}[1][\omega]{#1} % lettre pour une assignation de constantes
\newcommand{\Ome}[1][\Omega]{#1} % ensemble d'assignations de constantes
\newcommand{\Omei}[2][\Ome]{#1_{#2}} % ensemble d'assignations de constantes

\newcommand{\tet}[1][\theta]{#1} % lettre pour une assignation de variables
\newcommand{\Tet}[1][\Theta]{#1} % ensemble d'assignations de variables
\newcommand{\Teti}[2][\Tet]{#1_{#2}} % ensemble d'assignations de variables

\newcommand{\interCV}[3]{\|#3\|_{#1}^{#2}} % interpretation
\newcommand{\inter}[1]{\interCV{}{}{#1}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Macros pour les tableaux semantiques %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \coche[indice] insere une marke de coche indicee devant une formule
\newcommand{\coche}[1][]{\surd_{#1}\;\;}

% \tabvgap[vgap] sets the length of the vertical space between two
% consecutive nodes of the tableau-tree ; the default is 4mm  
\newcommand{\tabvgap}[1][3mm]{\setlength{\GapDepth}{#1}}

% \tabhgap[hgap] sets the length of the horizontal space between two
% adjacent nodes of the tableau-tree ; the default is 12mm  
\newcommand{\tabhgap}[1][1mm]{\setlength{\GapWidth}{#1}}

% \begin{tableau} ... \end{tableau} definit un environnement 
% de dessin d'un tableau semantique sous forme d'arbre binaire.
%\newenvironment{tableau}{\begin{array}{c}}{\end{array}}
\newenvironment{tableau}{}{}

% \tbloc[c|l|r]{lignes} regroupe plusieurs lignes en un bloc ;
% le parametre optionel permet de centrer ou de justifier les lignes
\newcommand{\tbloc}[1]{$\begin{array}{c} #1 \end{array}$}

\newcommand{\tclos}[1]{\tbloc{#1 \\ \times}}

% \tinfI{racine}{fils1}{fils2}
\newcommand{\tinfI}[4][0pt]
{\begin{bundle}{#2}
 \chunk{\tbloc{#3 \\ #4}}
 \end{bundle}
}

% \tinfIc{contrainte}{racine}{fils1}{fils2}
\newcommand{\tinfIc}[5][0pt]
{\begin{bundle}{#3}
 \chunk
 {
   \begin{bundle}{#2}
   \chunk{\tbloc{#4 \\ #5}}
   \end{bundle}
 }
 \end{bundle}
}

% \tinfII[espace_branches]{racine}{fils1}{fils2}
\newcommand{\tinfII}[4][2cm]
{\begin{bundle}{#2}
 \chunk
 { \begin{bundle}{}
   \chunk{\makebox[#1]{#3}}
   \chunk{\makebox[#1]{#4}}
   \end{bundle}
 }
 \end{bundle}
}

% \tinfIIc[espace_branches]{contrainte}{racine}{fils1}{fils2}
\newcommand{\tinfIIc}[5][2cm]
{\begin{bundle}{#3}
 \chunk
 { \begin{bundle}{#2}
   \chunk
   {
     \begin{bundle}{}
     \chunk{\makebox[#1]{#4}}
     \chunk{\makebox[#1]{#5}}
     \end{bundle}
   }
   \end{bundle}
 }
 \end{bundle}
}

% ajouts du 18/03/2001:

\newcommand{\Br}{\ett} % lettre pour une branche
\newcommand{\Tr}{{\cal T}} % lettre pour un arbe
\newcommand{\DG}{DG} % lettre pour un graphe de dependance
\newcommand{\garrowp}{\stackrel{\star}{\garrow}}
\newcommand{\Nod}{Nod}
\newcommand{\Arr}{Arr}

